An Improved Algorithm for Generating Database Transactions from Relational Algebra Specifications

Alloy is a lightweight modeling formalism based on relational algebra. In prior work with Fisler, Giannakopoulos, Krishnamurthi, and Yoo, we have presented a tool, Alchemy, that compiles Alloy specifications into implementations that execute against persistent databases. The foundation of Alchemy is an algorithm for rewriting relational algebra formulas into code for database transactions. In this paper we report on recent progress in improving the robustness and efficiency of this transformation.

==> R.Z0rule.tex <==
\begin{ZZZZschemedisplay}%
\HL \HL \HL \HL \HL \=\sy{sig} \va{Submission} \va{$\{$$\}$}\\%
     \>\sy{sig} \va{Grade} \va{$\{$$\}$}\\%
     \>\sy{sig} \va{Student} \va{$\{$$\}$}
\end{ZZZZschemedisplay}

\begin{ZZZZschemedisplay}%
\HL \HL \HL \HL \HL \sy{sig} \va{Course} \va{$\{$}\\%
\HL \HL \HL \HL \HL \HL \HL \=\va{roster} {\textrm :} \ \sy{set} \va{Student}, \\%
       \>\va{work} {\textrm :} \va{roster} $\rightarrow$ \va{Submission},\\%
       \>\va{gradebook} {\textrm :} \va{work} $\rightarrow$ \sy{lone} \va{Grade} \va{$\}$}
\end{ZZZZschemedisplay}

\begin{ZZZZschemedisplay}%
\HL \HL \HL \HL \HL \sy{pred} \va{Enroll} (\va{c}, \va{c}' {\textrm :} \va{Course}, \va{sNew} {\textrm :} \va{Student}) \va{$\{$}\\%
\HL \HL \HL \HL \HL \HL \HL \HL \=\va{c}'$$\va{.roster} \va{$=$} \va{c.roster} $\cup$ \va{sNew} \sy{and}\\%
        \>\va{c}'$$\va{.work}[\va{sNew}] \va{$=$} $\emptyset$ \va{$\}$}
\end{ZZZZschemedisplay}

\begin{ZZZZschemedisplay}%
\HL \HL \HL \HL \HL \sy{pred} \va{Drop} (\va{c}, \va{c}' {\textrm :} \va{Course}, \va{s:} \va{Student}) \va{$\{$}\\%
\HL \HL \HL \HL \HL \HL \HL \va{s} $\alloynotin$ \va{c}'$$\va{.roster} \va{$\}$}
\end{ZZZZschemedisplay}

\begin{ZZZZschemedisplay}%
\HL \HL \HL \HL \HL \sy{pred} \va{SubmitForPair} \=(\va{c}, \va{c}' {\textrm :} \va{Course}, \va{s1}, \va{s2} {\textrm :} \va{Student},\\%
                        \>\PRN \va{bNew} {\textrm :} \va{Submission}) \va{$\{$}\\%
\HL \HL \HL \HL \HL \HL \HL \=\va{//} $\mbox{pre-condition}$\\%
       \>\va{s1} $\alloyin$ \va{c.roster} \sy{and} \va{s2} $\alloyin$ \va{c.roster} \sy{and} \ \\%
       \>\va{//} $\mbox{update}$\\%
       \>\va{c}'$$\va{.work} \va{$=$} \va{c.work} $\cup$ \va{$\lt$s1}, \va{bNew$\gt$} $\cup$ \va{$\lt$s2}, \ \va{bNew$\gt$} \sy{and}\\%
       \>\va{//} $\mbox{frame condition}$\\%
       \>\va{c}'$$\va{.gradebook} \va{$=$} \va{c.gradebook} \va{$\}$}
\end{ZZZZschemedisplay}

\begin{ZZZZschemedisplay}%
\HL \HL \HL \HL \HL \sy{pred} \va{AssignGrade} \=(\va{c}, \va{c}' {\textrm :} \va{Course}, \va{s} {\textrm :} \va{Student}, \\%
                      \>\PRN \va{b} {\textrm :} \va{Submission}, \va{g} {\textrm :} \va{Grade}) \va{$\{$}\\%
\HL \HL \HL \HL \HL \HL \HL \=\va{c}'$$\va{.gradebook} $\alloyin$ \va{c.gradebook} $\cup$ \va{$\lt$s}, \ \va{b}, \va{g$\gt$} \sy{and}\\%
       \>\va{c}'$$\va{.roster} \va{$=$} \va{c.roster} \va{$\}$}
\end{ZZZZschemedisplay}

\begin{ZZZZschemedisplay}%
\HL \HL \HL \HL \HL \sy{fact} \va{SameGradeForPair} \va{$\{$}\\%
\HL \HL \HL \HL \HL \HL \HL \sy{all} \va{c} {\textrm :} \va{Course}, \va{s1}, \va{s2} {\textrm :} \va{Student}, \va{b} {\textrm :} \va{Submission} \va{$\vert$} \\%
\HL \HL \HL \HL \HL \HL \HL \HL \HL \HL \va{b} \sy{in} (\va{c.work}[\va{s1}] \cn{\&} \va{c.work}[\va{s2}]) \sy{implies}\\%
\HL \HL \HL \HL \HL \HL \HL \HL \HL \HL \HL \HL \HL \va{c.gradebook}[\va{s1}][\va{b}] \va{$=$} \va{c.gradebook}[\va{s2}][\va{b}] \va{$\}$}
\end{ZZZZschemedisplay}


==> R.Z10rule.tex <==
\ZZZZschemecodeintext
\va{Student}%
\endZZZZschemecodeintext


==> R.Z11rule.tex <==
\ZZZZschemecodeintext
\va{Submission}%
\endZZZZschemecodeintext


==> R.Z12rule.tex <==
\ZZZZschemecodeintext
\va{Course}%
\endZZZZschemecodeintext


==> R.Z13rule.tex <==
\ZZZZschemecodeintext
\va{Student}%
\endZZZZschemecodeintext


==> R.Z14rule.tex <==
\ZZZZschemecodeintext
\va{roster}%
\endZZZZschemecodeintext


==> R.Z15rule.tex <==
\ZZZZschemecodeintext
\sy{lone}%
\endZZZZschemecodeintext


==> R.Z16rule.tex <==
\ZZZZschemecodeintext
\va{gradebook}%
\endZZZZschemecodeintext


==> R.Z17rule.tex <==
\ZZZZschemecodeintext
\va{Enroll}%
\endZZZZschemecodeintext


==> R.Z18rule.tex <==
\ZZZZschemecodeintext
\va{c}%
\endZZZZschemecodeintext


==> R.Z19rule.tex <==
\ZZZZschemecodeintext
\va{c}'%
\endZZZZschemecodeintext


==> R.Z1rule.tex <==
\ZZZZschemecodeintext
\sy{sig}%
\endZZZZschemecodeintext


==> R.Z20rule.tex <==
\ZZZZschemecodeintext
\va{SameGradeForPair}%
\endZZZZschemecodeintext


==> R.Z21rule.tex <==
\ZZZZschemecodeintext
.%
\endZZZZschemecodeintext


==> R.Z22rule.tex <==
\begin{ZZZZschemedisplay}%
\HL \HL \HL \HL \HL \=\va{Student} \va{$=$} \va{$\{$Harry}, \va{Meg$\}$}\\%
     \>\va{Submission} \va{$=$} \va{$\{$hwk1$\}$}\\%
     \>\va{Grade} \va{$=$} \va{$\{$A}, $A-$, \va{B$+$}, \va{B$\}$}\\%
     \>\va{Course} \va{$=$} \va{$\{$c0}, \va{c1$\}$}\\%
     \>\va{roster} \va{$=$} ($\tuple{\scheme|c0, Harry|}$, $\tuple{\scheme|c1, Harry|}$, $\tuple{\scheme|c1, Meg|}$)\\%
     \>\va{work} \va{$=$} \va{$\{$}$\tuple{\scheme|c1, Harry, hwk1|}$\va{$\}$}\\%
     \>\va{gradebook} \va{$=$} \va{$\{$}$\tuple{\scheme|c1, Harry, hwk1, A-|}$\va{$\}$}
\end{ZZZZschemedisplay}


==> R.Z23rule.tex <==
\ZZZZschemecodeintext
\va{c0}, \va{Harry}%
\endZZZZschemecodeintext


==> R.Z24rule.tex <==
\ZZZZschemecodeintext
\va{c1}, \va{Harry}%
\endZZZZschemecodeintext


==> R.Z25rule.tex <==
\ZZZZschemecodeintext
\va{c1}, \va{Meg}%
\endZZZZschemecodeintext


==> R.Z26rule.tex <==
\ZZZZschemecodeintext
\va{c1}, \va{Harry}, \va{hwk1}%
\endZZZZschemecodeintext


==> R.Z27rule.tex <==
\ZZZZschemecodeintext
\va{c1}, \va{Harry}, \va{hwk1}, \va{A-}%
\endZZZZschemecodeintext


==> R.Z28rule.tex <==
\ZZZZschemecodeintext
\va{Enroll}%
\endZZZZschemecodeintext


==> R.Z29rule.tex <==
\ZZZZschemecodeintext
\va{c}%
\endZZZZschemecodeintext


==> R.Z2rule.tex <==
\ZZZZschemecodeintext
\va{Submission}%
\endZZZZschemecodeintext


==> R.Z30rule.tex <==
\ZZZZschemecodeintext
\va{c0}%
\endZZZZschemecodeintext


==> R.Z31rule.tex <==
\ZZZZschemecodeintext
\va{c}'%
\endZZZZschemecodeintext


==> R.Z32rule.tex <==
\ZZZZschemecodeintext
\va{c1}%
\endZZZZschemecodeintext


==> R.Z33rule.tex <==
\ZZZZschemecodeintext
\va{sNew}%
\endZZZZschemecodeintext


==> R.Z34rule.tex <==
\ZZZZschemecodeintext
\va{Meg}%
\endZZZZschemecodeintext


==> R.Z35rule.tex <==
\ZZZZschemecodeintext
\va{Enroll}%
\endZZZZschemecodeintext


==> R.Z36rule.tex <==
\ZZZZschemecodeintext
\va{work}%
\endZZZZschemecodeintext


==> R.Z37rule.tex <==
\ZZZZschemecodeintext
\va{c1}, \va{Harry}, \va{hwk1}%
\endZZZZschemecodeintext


==> R.Z38rule.tex <==
\ZZZZschemecodeintext
\va{work}%
\endZZZZschemecodeintext


==> R.Z39rule.tex <==
\ZZZZschemecodeintext
\va{SubmitForPair}%
\endZZZZschemecodeintext


==> R.Z3rule.tex <==
\ZZZZschemecodeintext
\sy{sig}%
\endZZZZschemecodeintext


==> R.Z40rule.tex <==
\ZZZZschemecodeintext
\va{SubmitForPair}%
\endZZZZschemecodeintext


==> R.Z41rule.tex <==
\ZZZZschemecodeintext
\va{c}%
\endZZZZschemecodeintext


==> R.Z42rule.tex <==
\ZZZZschemecodeintext
\va{c0}%
\endZZZZschemecodeintext


==> R.Z43rule.tex <==
\ZZZZschemecodeintext
\va{c}'%
\endZZZZschemecodeintext


==> R.Z44rule.tex <==
\ZZZZschemecodeintext
\va{c1}%
\endZZZZschemecodeintext


==> R.Z45rule.tex <==
\ZZZZschemecodeintext
\va{c}'%
\endZZZZschemecodeintext


==> R.Z46rule.tex <==
\ZZZZschemecodeintext
\va{.gradebook} \va{$=$} \va{c.gradebook}%
\endZZZZschemecodeintext


==> R.Z47rule.tex <==
\ZZZZschemecodeintext
\va{c}'%
\endZZZZschemecodeintext


==> R.Z48rule.tex <==
\ZZZZschemecodeintext
\va{c}%
\endZZZZschemecodeintext


==> R.Z49rule.tex <==
\ZZZZschemecodeintext
\va{work}%
\endZZZZschemecodeintext


==> R.Z4rule.tex <==
\ZZZZschemecodeintext
\va{Course}%
\endZZZZschemecodeintext


==> R.Z50rule.tex <==
\ZZZZschemecodeintext
\va{c}%
\endZZZZschemecodeintext


==> R.Z51rule.tex <==
\ZZZZschemecodeintext
\va{c}'%
\endZZZZschemecodeintext


==> R.Z52rule.tex <==
\ZZZZschemecodeintext
\va{Submission}%
\endZZZZschemecodeintext


==> R.Z53rule.tex <==
\ZZZZschemecodeintext
\va{roster}%
\endZZZZschemecodeintext


==> R.Z54rule.tex <==
\ZZZZschemecodeintext
\va{Enroll}%
\endZZZZschemecodeintext


==> R.Z55rule.tex <==
\ZZZZschemecodeintext
\va{CreateSubmission}%
\endZZZZschemecodeintext


==> R.Z56rule.tex <==
\begin{ZZZZschemedisplay}%
\HL \HL \HL \HL \HL \=\va{cs311} \va{$=$} \va{CreateCourse}(\dt{{\dq}cs311{\dq}});\\%
     \>\va{pete} \va{$=$} \va{CreateStudent}(\dt{{\dq}Pete{\dq}});\\%
     \>\va{caitlin} \va{$=$} \va{CreateStudent}(\dt{{\dq}Caitlin{\dq}});\\%
     \>\va{Enroll}(\va{cs311}, \va{pete});\\%
     \>\va{Enroll}(\va{cs311}, \va{caitlin})
\end{ZZZZschemedisplay}


==> R.Z57rule.tex <==
\ZZZZschemecodeintext
\va{Enroll}%
\endZZZZschemecodeintext


==> R.Z58rule.tex <==
\ZZZZschemecodeintext
\dt{{\dq}cs311{\dq}}%
\endZZZZschemecodeintext


==> R.Z59rule.tex <==
\ZZZZschemecodeintext
\dt{{\dq}Pete{\dq}}%
\endZZZZschemecodeintext


==> R.Z5rule.tex <==
\ZZZZschemecodeintext
\va{roster}%
\endZZZZschemecodeintext


==> R.Z60rule.tex <==
\ZZZZschemecodeintext
\dt{{\dq}cs311{\dq}}%
\endZZZZschemecodeintext


==> R.Z61rule.tex <==
\ZZZZschemecodeintext
\dt{{\dq}Caitlin{\dq}}%
\endZZZZschemecodeintext


==> R.Z62rule.tex <==
\ZZZZschemecodeintext
\va{roster}%
\endZZZZschemecodeintext


==> R.Z63rule.tex <==
\ZZZZschemecodeintext
\va{Enroll}%
\endZZZZschemecodeintext


==> R.Z64rule.tex <==
\ZZZZschemecodeintext
\va{work}%
\endZZZZschemecodeintext


==> R.Z65rule.tex <==
\ZZZZschemecodeintext
\dt{{\dq}Pete{\dq}}%
\endZZZZschemecodeintext


==> R.Z66rule.tex <==
\ZZZZschemecodeintext
\dt{{\dq}Caitlin{\dq}}%
\endZZZZschemecodeintext


==> R.Z67rule.tex <==
\begin{ZZZZschemedisplay}%
\HL \HL \HL \HL \HL \=\va{hwk1} \va{$=$} \va{CreateSubmission}(\dt{{\dq}hwk1{\dq}});\\%
     \>\va{SubmitForPair}(\va{cs311}, \va{pete}, \va{caitlin}, \va{hwk1})
\end{ZZZZschemedisplay}


==> R.Z68rule.tex <==
\ZZZZschemecodeintext
\va{SubmitForPair}%
\endZZZZschemecodeintext


==> R.Z69rule.tex <==
\ZZZZschemecodeintext
\va{work}%
\endZZZZschemecodeintext


==> R.Z6rule.tex <==
\ZZZZschemecodeintext
\va{Course}%
\endZZZZschemecodeintext


==> R.Z70rule.tex <==
\ZZZZschemecodeintext
\va{gradebook}%
\endZZZZschemecodeintext


==> R.Z71rule.tex <==
\begin{ZZZZschemedisplay}%
\HL \HL \HL \HL \HL \=\va{gradeA} \va{$=$} \va{CreateGrade}(\dt{{\dq}A{\dq}});\\%
     \>\va{AssignGrade}(\va{cs311}, \va{pete}, \va{hwk1}, \va{gradeA})
\end{ZZZZschemedisplay}


==> R.Z72rule.tex <==
\ZZZZschemecodeintext
\va{AssignGrade}%
\endZZZZschemecodeintext


==> R.Z73rule.tex <==
\ZZZZschemecodeintext
\va{gradebook}%
\endZZZZschemecodeintext


==> R.Z74rule.tex <==
\ZZZZschemecodeintext
\va{SameGradeForPair}%
\endZZZZschemecodeintext


==> R.Z75rule.tex <==
\ZZZZschemecodeintext
\dt{{\dq}Caitlin{\dq}}%
\endZZZZschemecodeintext


==> R.Z76rule.tex <==
\ZZZZschemecodeintext
\va{cs311}%
\endZZZZschemecodeintext


==> R.Z77rule.tex <==
\ZZZZschemecodeintext
\va{Caitlin}%
\endZZZZschemecodeintext


==> R.Z78rule.tex <==
\ZZZZschemecodeintext
\va{hwk1}%
\endZZZZschemecodeintext


==> R.Z79rule.tex <==
\ZZZZschemecodeintext
\va{A}%
\endZZZZschemecodeintext


==> R.Z7rule.tex <==
\ZZZZschemecodeintext
\va{Student}%
\endZZZZschemecodeintext


==> R.Z80rule.tex <==
\ZZZZschemecodeintext
\va{gradebook}%
\endZZZZschemecodeintext


==> R.Z81rule.tex <==
\ZZZZschemecodeintext
\va{SameGradeForPair}%
\endZZZZschemecodeintext


==> R.Z82rule.tex <==
\ZZZZschemecodeintext
\va{AssignGrade}%
\endZZZZschemecodeintext


==> R.Z83rule.tex <==
\begin{ZZZZschemedisplay}%
\HL \HL \HL \HL \HL \HL \=\cn{expr} \va{::$=$} \cn{rel} \va{$\vert$} \cn{var} \va{$\vert$} \cn{none} \va{$\vert$} \cn{expr} \cn{binop} \cn{expr} \va{$\vert$} \cn{unop} \cn{expr}\\%
      \>\cn{binop} \va{::$=$} $\cup$ \va{$\vert$} $\cap$ \va{$\vert$} $-$ \va{$\vert$} . \va{$\vert$} $\mthpair{}{}$\\%
      \>\cn{unop} \va{::$=$} \ $\sim$\va{$\vert$} $*$
\end{ZZZZschemedisplay}

\begin{ZZZZschemedisplay}%
\HL \HL \HL \HL \HL \HL \=\cn{formula} \va{::$=$} \cn{elemFormula} \va{$\vert$} \cn{compFormula} \va{$\vert$} \cn{quantFormula}\\%
      \>\cn{elemFormula} \va{::$=$} \cn{expr} $\alloyin$ \cn{expr} \va{$\vert$} \cn{expr} \va{$=$} \cn{expr} \ \\%
      \>\cn{compFormula} \va{::$=$} \sy{not} \cn{formula} \va{$\vert$} \cn{formula} $\land$ \cn{formula} \va{$\vert$} \cn{formula} $\lor$ \cn{formula}\\%
      \>\cn{quantFormula} \va{::$=$} $\forall$ \va{var:} \cn{expr} \va{$\{$} \cn{formula} \va{$\}$} \va{$\vert$} $\exists$ \va{var:} \cn{expr} \va{$\{$} \cn{formula} \va{$\}$}
\end{ZZZZschemedisplay}


==> R.Z8rule.tex <==
\ZZZZschemecodeintext
\va{work}%
\endZZZZschemecodeintext


==> R.Z9rule.tex <==
\ZZZZschemecodeintext
\va{Course}%
\endZZZZschemecodeintext


==> eptcsdata.tex <==
\providecommand{\event}{I. Mackie and A. Martins Moreira (Eds.): Tenth International\\Workshop on Rule-Based Programming (RULE 2009)}
\providecommand{\volume}{21}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{77}
\providecommand{\eid}{7}

